Weak lensing combined with the kinetic Sunyaev Zel'dovich effect: A study of baryonic feedback

Extracting precise cosmology from weak lensing surveys requires modelling the non-linear matter power spectrum, which is suppressed at small scales due to baryonic feedback processes. However, hydrodynamical galaxy formation simulations make widely varying predictions for the amplitude and extent of this effect. We use measurements of Dark Energy Survey Year 3 weak lensing (WL) and Atacama Cosmology Telescope DR5 kinematic Sunyaev-Zel'dovich (kSZ) to jointly constrain cosmological and astrophysical baryonic feedback parameters using a flexible analytical model, `baryonification'. First, using WL only, we compare the $S_8$ constraints using baryonification to a simulation-calibrated halo model, a simulation-based emulator model and the approach of discarding WL measurements on small angular scales. We find that model flexibility can shift the value of $S_8$ and degrade the uncertainty. The kSZ provides additional constraints on the astrophysical parameters and shifts $S_8$ to $S_8=0.823^{+0.019}_{-0.020}$, a higher value than attained using the WL-only analysis. We measure the suppression of the non-linear matter power spectrum using WL + kSZ and constrain a mean feedback scenario that is more extreme than the predictions from most hydrodynamical simulations. We constrain the baryon fractions and the gas mass fractions and find them to be generally lower than inferred from X-ray observations and simulation predictions. We conclude that the WL + kSZ measurements provide a new and complementary benchmark for building a coherent picture of the impact of gas around galaxies across observations.

==> author_list_fin.tex <==
% Author list file generated with: mkauthlist.py 1.3.0+14.gcc6daf1 
% mkauthlist.py --sort-builder --aux /home/lmb224/Notebooks/firstauthors.csv /home/lmb224/Notebooks/DES_author_list.csv author_list_fin.tex 

\author{L.~Bigwood}
\affiliation{Institute of Astronomy, University of Cambridge, Madingley Road, Cambridge CB3 0HA, UK}

\author{A.~Amon}
\affiliation{Department of Astrophysical Sciences, Princeton University, Peyton Hall, Princeton, NJ 08544, USA}

\author{A.~Schneider}
\affiliation{Institute for Computational Science, University of Zurich, Winterthurerstrasse 190, CH-8057 Zurich, Switzerland}

\author{J.~Salcido}
\affiliation{Astrophysics Research Institute, Liverpool John Moores University, 146 Brownlow Hill, Liverpool L3 5RF, UK}

\author{I.~G.~McCarthy}
\affiliation{Astrophysics Research Institute, Liverpool John Moores University, 146 Brownlow Hill, Liverpool L3 5RF, UK}

\author{A.~Roodman}
\affiliation{Kavli Institute for Particle Astrophysics \& Cosmology, P. O. Box 2450, Stanford University, Stanford, CA 94305, USA}
\affiliation{SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA}

\author{A.~Pieres}
\affiliation{Laborat\'orio Interinstitucional de e-Astronomia - LIneA, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil}
\affiliation{Observat\'orio Nacional, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil}

\author{A.~Fert\'e}
\affiliation{SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA}

\author{A.~Alarcon}
\affiliation{Argonne National Laboratory, 9700 South Cass Avenue, Lemont, IL 60439, USA}
\affiliation{Institute of Space Sciences (ICE, CSIC),  Campus UAB, Carrer de Can Magrans, s/n,  08193 Barcelona, Spain}

\author{A.~Drlica-Wagner}
\affiliation{Department of Astronomy and Astrophysics, University of Chicago, Chicago, IL 60637, USA}
\affiliation{Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA}
\affiliation{Kavli Institute for Cosmological Physics, University of Chicago, Chicago, IL 60637, USA}

\author{A.~Choi}
\affiliation{NASA Goddard Space Flight Center, 8800 Greenbelt Rd, Greenbelt, MD 20771, USA}

\author{A. Navarro-Alsina}
\affiliation{Instituto de F\'isica Gleb Wataghin, Universidade Estadual de Campinas, 13083-859, Campinas, SP, Brazil}

\author{A.~Campos}
\affiliation{Department of Physics, Carnegie Mellon University, Pittsburgh, Pennsylvania 15312, USA}
\affiliation{NSF AI Planning Institute for Physics of the Future, Carnegie Mellon University, Pittsburgh, PA 15213, USA}

\author{A.~Chen}
\affiliation{Department of Physics, University of Michigan, Ann Arbor, MI 48109, USA}
\affiliation{Kavli Institute for the Physics and Mathematics of the Universe (WPI), UTIAS, The University of Tokyo, Kashiwa, Chiba 277-8583, Japan}

\author{A.~J.~Ross}
\affiliation{Center for Cosmology and Astro-Particle Physics, The Ohio State University, Columbus, OH 43210, USA}

\author{A.~Carnero~Rosell}
\affiliation{Instituto de Astrofisica de Canarias, E-38205 La Laguna, Tenerife, Spain}
\affiliation{Laborat\'orio Interinstitucional de e-Astronomia - LIneA, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil}

\author{B.~Yin}
\affiliation{Department of Physics, Carnegie Mellon University, Pittsburgh, Pennsylvania 15312, USA}

\author{B.~Yanny}
\affiliation{Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA}

\author{C.~S{\'a}nchez}
\affiliation{Department of Physics and Astronomy, University of Pennsylvania, Philadelphia, PA 19104, USA}

\author{C.~Chang}
\affiliation{Department of Astronomy and Astrophysics, University of Chicago, Chicago, IL 60637, USA}
\affiliation{Kavli Institute for Cosmological Physics, University of Chicago, Chicago, IL 60637, USA}

\author{C.~Davis}
\affiliation{Kavli Institute for Particle Astrophysics \& Cosmology, P. O. Box 2450, Stanford University, Stanford, CA 94305, USA}

\author{C.~Doux}
\affiliation{Department of Physics and Astronomy, University of Pennsylvania, Philadelphia, PA 19104, USA}
\affiliation{Universit\'e Grenoble Alpes, CNRS, LPSC-IN2P3, 38000 Grenoble, France}

\author{D.~Gruen}
\affiliation{University Observatory, Faculty of Physics, Ludwig-Maximilians-Universit\"at, Scheinerstr. 1, 81679 Munich, Germany}

\author{E.~S.~Rykoff}
\affiliation{Kavli Institute for Particle Astrophysics \& Cosmology, P. O. Box 2450, Stanford University, Stanford, CA 94305, USA}
\affiliation{SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA}

\author{E.~Krause}
\affiliation{Department of Astronomy/Steward Observatory, University of Arizona, 933 North Cherry Avenue, Tucson, AZ 85721-0065, USA}

\author{E.~M.~Huff}
\affiliation{Jet Propulsion Laboratory, California Institute of Technology, 4800 Oak Grove Dr., Pasadena, CA 91109, USA}

\author{E.~Sheldon}
\affiliation{Brookhaven National Laboratory, Bldg 510, Upton, NY 11973, USA}

\author{F.~Tarsitano}
\affiliation{Department of Physics, ETH Zurich, Wolfgang-Pauli-Strasse 16, CH-8093 Zurich, Switzerland}

\author{F.~Andrade-Oliveira}
\affiliation{Department of Physics, University of Michigan, Ann Arbor, MI 48109, USA}

\author{G.~M.~Bernstein}
\affiliation{Department of Physics and Astronomy, University of Pennsylvania, Philadelphia, PA 19104, USA}

\author{G.~Giannini}
\affiliation{Institut de F\'{\i}sica d'Altes Energies (IFAE), The Barcelona Institute of Science and Technology, Campus UAB, 08193 Bellaterra (Barcelona) Spain}
\affiliation{Kavli Institute for Cosmological Physics, University of Chicago, Chicago, IL 60637, USA}

\author{H.~T.~Diehl}
\affiliation{Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA}

\author{H.~Huang}
\affiliation{Department of Astronomy/Steward Observatory, University of Arizona, 933 North Cherry Avenue, Tucson, AZ 85721-0065, USA}
\affiliation{Department of Physics, University of Arizona, Tucson, AZ 85721, USA}

\author{I.~Harrison}
\affiliation{School of Physics and Astronomy, Cardiff University, CF24 3AA, UK}

\author{I.~Sevilla-Noarbe}
\affiliation{Centro de Investigaciones Energ\'eticas, Medioambientales y Tecnol\'ogicas (CIEMAT), Madrid, Spain}

\author{I.~Tutusaus}
\affiliation{Institut de Recherche en Astrophysique et Plan\'etologie (IRAP), Universit\'e de Toulouse, CNRS, UPS, CNES, 14 Av. Edouard Belin, 31400 Toulouse, France}

\author{J.~Elvin-Poole}
\affiliation{Department of Physics and Astronomy, University of Waterloo, 200 University Ave W, Waterloo, ON N2L 3G1, Canada}

\author{J.~McCullough}
\affiliation{Kavli Institute for Particle Astrophysics \& Cosmology, P. O. Box 2450, Stanford University, Stanford, CA 94305, USA}

\author{J.~Zuntz}
\affiliation{Institute for Astronomy, University of Edinburgh, Edinburgh EH9 3HJ, UK}

\author{J.~Blazek}
\affiliation{Department of Physics, Northeastern University, Boston, MA 02115, USA}

\author{J.~DeRose}
\affiliation{Lawrence Berkeley National Laboratory, 1 Cyclotron Road, Berkeley, CA 94720, USA}

\author{J.~Cordero}
\affiliation{Jodrell Bank Center for Astrophysics, School of Physics and Astronomy, University of Manchester, Oxford Road, Manchester, M13 9PL, UK}

\author{J.~Prat}
\affiliation{Department of Astronomy and Astrophysics, University of Chicago, Chicago, IL 60637, USA}
\affiliation{Nordita, KTH Royal Institute of Technology and Stockholm University, Hannes Alfv\'ens v\"ag 12, SE-10691 Stockholm, Sweden}

\author{J.~Myles}
\affiliation{Department of Astrophysical Sciences, Princeton University, Peyton Hall, Princeton, NJ 08544, USA}

\author{K.~Eckert}
\affiliation{Department of Physics and Astronomy, University of Pennsylvania, Philadelphia, PA 19104, USA}

\author{K.~Bechtol}
\affiliation{Physics Department, 2320 Chamberlin Hall, University of Wisconsin-Madison, 1150 University Avenue Madison, WI  53706-1390}

\author{K.~Herner}
\affiliation{Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA}

\author{L.~F.~Secco}
\affiliation{Kavli Institute for Cosmological Physics, University of Chicago, Chicago, IL 60637, USA}

\author{M.~Gatti}
\affiliation{Department of Physics and Astronomy, University of Pennsylvania, Philadelphia, PA 19104, USA}

\author{M.~Raveri}
\affiliation{Department of Physics, University of Genova and INFN, Via Dodecaneso 33, 16146, Genova, Italy}

\author{M.~Carrasco~Kind}
\affiliation{Center for Astrophysical Surveys, National Center for Supercomputing Applications, 1205 West Clark St., Urbana, IL 61801, USA}
\affiliation{Department of Astronomy, University of Illinois at Urbana-Champaign, 1002 W. Green Street, Urbana, IL 61801, USA}

\author{M.~R.~Becker}
\affiliation{Argonne National Laboratory, 9700 South Cass Avenue, Lemont, IL 60439, USA}

\author{M.~A.~Troxel}
\affiliation{Department of Physics, Duke University Durham, NC 27708, USA}

\author{M.~Jarvis}
\affiliation{Department of Physics and Astronomy, University of Pennsylvania, Philadelphia, PA 19104, USA}

\author{N.~MacCrann}
\affiliation{Department of Applied Mathematics and Theoretical Physics, University of Cambridge, Cambridge CB3 0WA, UK}

\author{O.~Friedrich}
\affiliation{Kavli Institute for Cosmology, University of Cambridge, Madingley Road, Cambridge CB3 0HA, UK}

\author{O.~Alves}
\affiliation{Department of Physics, University of Michigan, Ann Arbor, MI 48109, USA}

\author{P.-F.~Leget}
\affiliation{Kavli Institute for Particle Astrophysics \& Cosmology, P. O. Box 2450, Stanford University, Stanford, CA 94305, USA}

\author{R.~Chen}
\affiliation{Department of Physics, Duke University Durham, NC 27708, USA}

\author{R.~P.~Rollins}
\affiliation{Jodrell Bank Center for Astrophysics, School of Physics and Astronomy, University of Manchester, Oxford Road, Manchester, M13 9PL, UK}

\author{R.~H.~Wechsler}
\affiliation{Department of Physics, Stanford University, 382 Via Pueblo Mall, Stanford, CA 94305, USA}
\affiliation{Kavli Institute for Particle Astrophysics \& Cosmology, P. O. Box 2450, Stanford University, Stanford, CA 94305, USA}
\affiliation{SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA}

\author{R.~A.~Gruendl}
\affiliation{Center for Astrophysical Surveys, National Center for Supercomputing Applications, 1205 West Clark St., Urbana, IL 61801, USA}
\affiliation{Department of Astronomy, University of Illinois at Urbana-Champaign, 1002 W. Green Street, Urbana, IL 61801, USA}

\author{R.~Cawthon}
\affiliation{Physics Department, William Jewell College, Liberty, MO, 64068}

\author{S.~L.~Bridle}
\affiliation{Jodrell Bank Center for Astrophysics, School of Physics and Astronomy, University of Manchester, Oxford Road, Manchester, M13 9PL, UK}

\author{S.~Dodelson}
\affiliation{Department of Physics, Carnegie Mellon University, Pittsburgh, Pennsylvania 15312, USA}
\affiliation{NSF AI Planning Institute for Physics of the Future, Carnegie Mellon University, Pittsburgh, PA 15213, USA}

\author{S.~Pandey}
\affiliation{Department of Physics and Astronomy, University of Pennsylvania, Philadelphia, PA 19104, USA}

\author{S.~Everett}
\affiliation{Jet Propulsion Laboratory, California Institute of Technology, 4800 Oak Grove Dr., Pasadena, CA 91109, USA}

\author{T.~Shin}
\affiliation{Department of Physics and Astronomy, Stony Brook University, Stony Brook, NY 11794, USA}

\author{W.~G.~Hartley}
\affiliation{Department of Astronomy, University of Geneva, ch. d'\'Ecogia 16, CH-1290 Versoix, Switzerland}

\author{X.~Fang}
\affiliation{Department of Astronomy, University of California, Berkeley,  501 Campbell Hall, Berkeley, CA 94720, USA}
\affiliation{Department of Astronomy/Steward Observatory, University of Arizona, 933 North Cherry Avenue, Tucson, AZ 85721-0065, USA}

\author{Y.~Zhang}
\affiliation{Cerro Tololo Inter-American Observatory, NSF's National Optical-Infrared Astronomy Research Laboratory, Casilla 603, La Serena, Chile}

\author{(DES Collaboration)}

\collaboration{(DES Collaboration)}


==> author_list_mnras_final.tex <==
% Author list file generated with: mkauthlist.py 1.3.0+14.gcc6daf1 
% mkauthlist.py -j mnras --sort-builder --aux /home/lmb224/Notebooks/firstauthors.csv /home/lmb224/Notebooks/DES-2024-0827_author_list_fin.csv author_list_mnras_final.tex 

\author[DES Collaboration]{
\parbox{\textwidth}{
\Large
L.~Bigwood,$^{1,2}$
A.~Amon,$^{3,1,2}$
A.~Schneider,$^{4}$
J.~Salcido,$^{5}$
I.~G.~McCarthy,$^{5}$
C.~Preston,$^{1}$
D.~Sanchez,$^{6}$
D.~Sijacki,$^{1,2}$
E.~Schaan,$^{7,8}$
S.~Ferraro,$^{9,10}$
N.~Battaglia,$^{11}$
S.~Dodelson,$^{12,13}$
A.~Roodman,$^{14,15}$
A.~Pieres,$^{16,17}$
A.~Fert\'e,$^{15}$
A.~Alarcon,$^{18,19}$
A.~Drlica-Wagner,$^{20,21,22}$
A.~Choi,$^{23}$
A. Navarro-Alsina,$^{24}$
A.~Campos,$^{12,13}$
A.~Chen,$^{25,26}$
A.~J.~Ross,$^{27}$
A.~Carnero~Rosell,$^{28,16}$
B.~Yin,$^{12}$
B.~Yanny,$^{21}$
C.~S{\'a}nchez,$^{29}$
C.~Chang,$^{20,22}$
C.~Davis,$^{14}$
C.~Doux,$^{29,30}$
D.~Gruen,$^{31}$
E.~S.~Rykoff,$^{14,15}$
E.~M.~Huff,$^{32}$
E.~Sheldon,$^{33}$
F.~Tarsitano,$^{34}$
F.~Andrade-Oliveira,$^{25}$
G.~M.~Bernstein,$^{29}$
G.~Giannini,$^{35,22}$
H.~T.~Diehl,$^{21}$
H.~Huang,$^{36,37}$
I.~Harrison,$^{38}$
I.~Sevilla-Noarbe,$^{39}$
I.~Tutusaus,$^{40}$
J.~Elvin-Poole,$^{41}$
J.~McCullough,$^{14}$
J.~Zuntz,$^{42}$
J.~Blazek,$^{43}$
J.~DeRose,$^{44}$
J.~Cordero,$^{45}$
J.~Prat,$^{20,46}$
J.~Myles,$^{3}$
K.~Eckert,$^{29}$
K.~Bechtol,$^{47}$
K.~Herner,$^{21}$
L.~F.~Secco,$^{22}$
M.~Gatti,$^{29}$
M.~Raveri,$^{48}$
M.~Carrasco~Kind,$^{49,50}$
M.~R.~Becker,$^{18}$
M.~A.~Troxel,$^{51}$
M.~Jarvis,$^{29}$
N.~MacCrann,$^{52}$
O.~Friedrich,$^{53}$
O.~Alves,$^{25}$
P.-F.~Leget,$^{14}$
R.~Chen,$^{51}$
R.~P.~Rollins,$^{45}$
R.~H.~Wechsler,$^{54,14,15}$
R.~A.~Gruendl,$^{49,50}$
R.~Cawthon,$^{55}$
S.~Allam,$^{21}$
S.~L.~Bridle,$^{45}$
S.~Pandey,$^{29}$
S.~Everett,$^{32}$
T.~Shin,$^{56}$
W.~G.~Hartley,$^{57}$
X.~Fang,$^{58,36}$
Y.~Zhang,$^{59}$
M.~Aguena,$^{16}$
J.~Annis,$^{21}$
D.~Bacon,$^{60}$
E.~Bertin,$^{61,62}$
S.~Bocquet,$^{31}$
D.~Brooks,$^{63}$
J.~Carretero,$^{35}$
F.~J.~Castander,$^{64,19}$
L.~N.~da Costa,$^{16}$
M.~E.~S.~Pereira,$^{65}$
J.~De~Vicente,$^{39}$
S.~Desai,$^{66}$
P.~Doel,$^{63}$
I.~Ferrero,$^{67}$
B.~Flaugher,$^{21}$
J.~Frieman,$^{21,22}$
J.~Garc\'ia-Bellido,$^{68}$
E.~Gaztanaga,$^{64,60,19}$
G.~Gutierrez,$^{21}$
S.~R.~Hinton,$^{69}$
D.~L.~Hollowood,$^{70}$
K.~Honscheid,$^{27,71}$
D.~Huterer,$^{25}$
D.~J.~James,$^{72}$
K.~Kuehn,$^{73,74}$
O.~Lahav,$^{63}$
S.~Lee,$^{32}$
J.~L.~Marshall,$^{75}$
J. Mena-Fern{\'a}ndez,$^{76}$
R.~Miquel,$^{77,35}$
J.~Muir,$^{78}$
M.~Paterno,$^{21}$
A.~A.~Plazas~Malag\'on,$^{14,15}$
A.~Porredon,$^{79}$
A.~K.~Romer,$^{80}$
S.~Samuroff,$^{43}$
E.~Sanchez,$^{39}$
D.~Sanchez Cid,$^{39}$
M.~Smith,$^{81}$
M.~Soares-Santos,$^{82,25}$
E.~Suchyta,$^{83}$
M.~E.~C.~Swanson,$^{49}$
G.~Tarle,$^{25}$
C.~To,$^{27}$
N.~Weaverdyck,$^{58,44}$
J.~Weller,$^{84,85}$
P.~Wiseman,$^{81}$
and M.~Yamamoto$^{51}$
\begin{center} (DES Collaboration) \end{center}
}
\vspace{0.4cm}
\\
\parbox{\textwidth}{
%\scriptsize
$^{1}$ Institute of Astronomy, University of Cambridge, Madingley Road, Cambridge CB3 0HA, UK\\
$^{2}$ Kavli Institute for Cosmology Cambridge, Madingley Road, Cambridge, CB3 OHA\\
$^{3}$ Department of Astrophysical Sciences, Princeton University, Peyton Hall, Princeton, NJ 08544, USA\\
$^{4}$ Institute for Computational Science, University of Zurich, Winterthurerstrasse 190, CH-8057 Zurich, Switzerland\\
$^{5}$ Astrophysics Research Institute, Liverpool John Moores University, 146 Brownlow Hill, Liverpool L3 5RF, UK\\
$^{6}$ Centre for Energy, Environmental and Technological Research, Av. Complutense, 40, Moncloa - Aravaca, 28040 Madrid, Spain\\
$^{7}$ Kavli Institute for Particle Astrophysics and Cosmology,
382 Via Pueblo Mall Stanford, CA 94305-4060, USA\\
$^{8}$ SLAC National Accelerator Laboratory 2575 Sand Hill Road Menlo Park, California 94025, USA\\
$^{9}$ Physics Division, Lawrence Berkeley National Laboratory, Berkeley, CA 94720, USA\\
$^{10}$ Berkeley Center for Cosmological Physics, Department of Physics,
University of California, Berkeley, CA 94720, USA\\
$^{11}$  Department of Astronomy, Cornell University, Ithaca, NY 14853, USA\\
$^{12}$ Department of Physics, Carnegie Mellon University, Pittsburgh, Pennsylvania 15312, USA\\
$^{13}$ NSF AI Planning Institute for Physics of the Future, Carnegie Mellon University, Pittsburgh, PA 15213, USA\\
$^{14}$ Kavli Institute for Particle Astrophysics \& Cosmology, P. O. Box 2450, Stanford University, Stanford, CA 94305, USA\\
$^{15}$ SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA\\
$^{16}$ Laborat\'orio Interinstitucional de e-Astronomia - LIneA, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil\\
$^{17}$ Observat\'orio Nacional, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil\\
$^{18}$ Argonne National Laboratory, 9700 South Cass Avenue, Lemont, IL 60439, USA\\
$^{19}$ Institute of Space Sciences (ICE, CSIC),  Campus UAB, Carrer de Can Magrans, s/n,  08193 Barcelona, Spain\\
$^{20}$ Department of Astronomy and Astrophysics, University of Chicago, Chicago, IL 60637, USA\\
$^{21}$ Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA\\
$^{22}$ Kavli Institute for Cosmological Physics, University of Chicago, Chicago, IL 60637, USA\\
$^{23}$ NASA Goddard Space Flight Center, 8800 Greenbelt Rd, Greenbelt, MD 20771, USA\\
$^{24}$ Instituto de F\'isica Gleb Wataghin, Universidade Estadual de Campinas, 13083-859, Campinas, SP, Brazil\\
$^{25}$ Department of Physics, University of Michigan, Ann Arbor, MI 48109, USA\\
$^{26}$ Kavli Institute for the Physics and Mathematics of the Universe (WPI), UTIAS, The University of Tokyo, Kashiwa, Chiba 277-8583, Japan\\
$^{27}$ Center for Cosmology and Astro-Particle Physics, The Ohio State University, Columbus, OH 43210, USA\\
$^{28}$ Instituto de Astrofisica de Canarias, E-38205 La Laguna, Tenerife, Spain\\
$^{29}$ Department of Physics and Astronomy, University of Pennsylvania, Philadelphia, PA 19104, USA\\
$^{30}$ Universit\'e Grenoble Alpes, CNRS, LPSC-IN2P3, 38000 Grenoble, France\\
$^{31}$ University Observatory, Faculty of Physics, Ludwig-Maximilians-Universit\"at, Scheinerstr. 1, 81679 Munich, Germany\\
$^{32}$ Jet Propulsion Laboratory, California Institute of Technology, 4800 Oak Grove Dr., Pasadena, CA 91109, USA\\
$^{33}$ Brookhaven National Laboratory, Bldg 510, Upton, NY 11973, USA\\
$^{34}$ Department of Physics, ETH Zurich, Wolfgang-Pauli-Strasse 16, CH-8093 Zurich, Switzerland\\
$^{35}$ Institut de F\'{\i}sica d'Altes Energies (IFAE), The Barcelona Institute of Science and Technology, Campus UAB, 08193 Bellaterra (Barcelona) Spain\\
$^{36}$ Department of Astronomy/Steward Observatory, University of Arizona, 933 North Cherry Avenue, Tucson, AZ 85721-0065, USA\\
$^{37}$ Department of Physics, University of Arizona, Tucson, AZ 85721, USA\\
$^{38}$ School of Physics and Astronomy, Cardiff University, CF24 3AA, UK\\
$^{39}$ Centro de Investigaciones Energ\'eticas, Medioambientales y Tecnol\'ogicas (CIEMAT), Madrid, Spain\\
$^{40}$ Institut de Recherche en Astrophysique et Plan\'etologie (IRAP), Universit\'e de Toulouse, CNRS, UPS, CNES, 14 Av. Edouard Belin, 31400 Toulouse, France\\
$^{41}$ Department of Physics and Astronomy, University of Waterloo, 200 University Ave W, Waterloo, ON N2L 3G1, Canada\\
$^{42}$ Institute for Astronomy, University of Edinburgh, Edinburgh EH9 3HJ, UK\\
$^{43}$ Department of Physics, Northeastern University, Boston, MA 02115, USA\\
$^{44}$ Lawrence Berkeley National Laboratory, 1 Cyclotron Road, Berkeley, CA 94720, USA\\
$^{45}$ Jodrell Bank Center for Astrophysics, School of Physics and Astronomy, University of Manchester, Oxford Road, Manchester, M13 9PL, UK\\
$^{46}$ Nordita, KTH Royal Institute of Technology and Stockholm University, Hannes Alfv\'ens v\"ag 12, SE-10691 Stockholm, Sweden\\
$^{47}$ Physics Department, 2320 Chamberlin Hall, University of Wisconsin-Madison, 1150 University Avenue Madison, WI  53706-1390\\
$^{48}$ Department of Physics, University of Genova and INFN, Via Dodecaneso 33, 16146, Genova, Italy\\
$^{49}$ Center for Astrophysical Surveys, National Center for Supercomputing Applications, 1205 West Clark St., Urbana, IL 61801, USA\\
$^{50}$ Department of Astronomy, University of Illinois at Urbana-Champaign, 1002 W. Green Street, Urbana, IL 61801, USA\\
$^{51}$ Department of Physics, Duke University Durham, NC 27708, USA\\
$^{52}$ Department of Applied Mathematics and Theoretical Physics, University of Cambridge, Cambridge CB3 0WA, UK\\
$^{53}$ Kavli Institute for Cosmology, University of Cambridge, Madingley Road, Cambridge CB3 0HA, UK\\
$^{54}$ Department of Physics, Stanford University, 382 Via Pueblo Mall, Stanford, CA 94305, USA\\
$^{55}$ Physics Department, William Jewell College, Liberty, MO, 64068\\
$^{56}$ Department of Physics and Astronomy, Stony Brook University, Stony Brook, NY 11794, USA\\
$^{57}$ Department of Astronomy, University of Geneva, ch. d'\'Ecogia 16, CH-1290 Versoix, Switzerland\\
$^{58}$ Department of Astronomy, University of California, Berkeley,  501 Campbell Hall, Berkeley, CA 94720, USA\\
$^{59}$ Cerro Tololo Inter-American Observatory, NSF's National Optical-Infrared Astronomy Research Laboratory, Casilla 603, La Serena, Chile\\
$^{60}$ Institute of Cosmology and Gravitation, University of Portsmouth, Portsmouth, PO1 3FX, UK\\
$^{61}$ CNRS, UMR 7095, Institut d'Astrophysique de Paris, F-75014, Paris, France\\
$^{62}$ Sorbonne Universit\'es, UPMC Univ Paris 06, UMR 7095, Institut d'Astrophysique de Paris, F-75014, Paris, France\\
$^{63}$ Department of Physics \& Astronomy, University College London, Gower Street, London, WC1E 6BT, UK\\
$^{64}$ Institut d'Estudis Espacials de Catalunya (IEEC), 08034 Barcelona, Spain\\
$^{65}$ Hamburger Sternwarte, Universit\"{a}t Hamburg, Gojenbergsweg 112, 21029 Hamburg, Germany\\
$^{66}$ Department of Physics, IIT Hyderabad, Kandi, Telangana 502285, India\\
$^{67}$ Institute of Theoretical Astrophysics, University of Oslo. P.O. Box 1029 Blindern, NO-0315 Oslo, Norway\\
$^{68}$ Instituto de Fisica Teorica UAM/CSIC, Universidad Autonoma de Madrid, 28049 Madrid, Spain\\
$^{69}$ School of Mathematics and Physics, University of Queensland,  Brisbane, QLD 4072, Australia\\
$^{70}$ Santa Cruz Institute for Particle Physics, Santa Cruz, CA 95064, USA\\
$^{71}$ Department of Physics, The Ohio State University, Columbus, OH 43210, USA\\
$^{72}$ Center for Astrophysics $\vert$ Harvard \& Smithsonian, 60 Garden Street, Cambridge, MA 02138, USA\\
$^{73}$ Australian Astronomical Optics, Macquarie University, North Ryde, NSW 2113, Australia\\
$^{74}$ Lowell Observatory, 1400 Mars Hill Rd, Flagstaff, AZ 86001, USA\\
$^{75}$ George P. and Cynthia Woods Mitchell Institute for Fundamental Physics and Astronomy, and Department of Physics and Astronomy, Texas A\&M University, College Station, TX 77843,  USA\\
$^{76}$ LPSC Grenoble - 53, Avenue des Martyrs 38026 Grenoble, France\\
$^{77}$ Instituci\'o Catalana de Recerca i Estudis Avan\c{c}ats, E-08010 Barcelona, Spain\\
$^{78}$ Perimeter Institute for Theoretical Physics, 31 Caroline St. North, Waterloo, ON N2L 2Y5, Canada\\
$^{79}$ Ruhr University Bochum, Faculty of Physics and Astronomy, Astronomical Institute, German Centre for Cosmological Lensing, 44780 Bochum, Germany\\
$^{80}$ Department of Physics and Astronomy, Pevensey Building, University of Sussex, Brighton, BN1 9QH, UK\\
$^{81}$ School of Physics and Astronomy, University of Southampton,  Southampton, SO17 1BJ, UK\\
$^{82}$ \\
$^{83}$ Computer Science and Mathematics Division, Oak Ridge National Laboratory, Oak Ridge, TN 37831\\
$^{84}$ Max Planck Institute for Extraterrestrial Physics, Giessenbachstrasse, 85748 Garching, Germany\\
$^{85}$ Universit\"ats-Sternwarte, Fakult\"at f\"ur Physik, Ludwig-Maximilians Universit\"at M\"unchen, Scheinerstr. 1, 81679 M\"unchen, Germany\\
}
}


==> author_list_mnras_final2.tex <==
% Author list file generated with: mkauthlist.py 1.3.0+14.gcc6daf1 
% mkauthlist.py -j mnras --sort-builder --aux /home/lmb224/Notebooks/firstauthors.csv /home/lmb224/Notebooks/DES-2024-0827_author_list_fin.csv author_list_mnras_final2.tex 

\author[DES Collaboration]{
\parbox{\textwidth}{
\Large
L.~Bigwood,$^{1,2}$
A.~Amon,$^{3,1,2}$
A.~Schneider,$^{4}$
J.~Salcido,$^{5}$
I.~G.~McCarthy,$^{5}$
C.~Preston,$^{1}$
D.~Sanchez,$^{6}$
D.~Sijacki,$^{1,2}$
E.~Schaan,$^{7,8}$
S.~Ferraro,$^{9,10}$
N.~Battaglia,$^{11}$
A.~Chen,$^{12,13}$
S.~Dodelson,$^{14,15}$
A.~Roodman,$^{16,17}$
A.~Pieres,$^{18,19}$
A.~Fert\'e,$^{17}$
A.~Alarcon,$^{20,21}$
A.~Drlica-Wagner,$^{22,23,24}$
A.~Choi,$^{25}$
A. Navarro-Alsina,$^{26}$
A.~Campos,$^{14,15}$
A.~J.~Ross,$^{27}$
A.~Carnero~Rosell,$^{28,18}$
B.~Yin,$^{14}$
B.~Yanny,$^{23}$
C.~S{\'a}nchez,$^{29}$
C.~Chang,$^{22,24}$
C.~Davis,$^{16}$
C.~Doux,$^{29,30}$
D.~Gruen,$^{31}$
E.~S.~Rykoff,$^{16,17}$
E.~M.~Huff,$^{32}$
E.~Sheldon,$^{33}$
F.~Tarsitano,$^{34}$
F.~Andrade-Oliveira,$^{12}$
G.~M.~Bernstein,$^{29}$
G.~Giannini,$^{35,24}$
H.~T.~Diehl,$^{23}$
H.~Huang,$^{36,37}$
I.~Harrison,$^{38}$
I.~Sevilla-Noarbe,$^{39}$
I.~Tutusaus,$^{40}$
J.~Elvin-Poole,$^{41}$
J.~McCullough,$^{16}$
J.~Zuntz,$^{42}$
J.~Blazek,$^{43}$
J.~DeRose,$^{44}$
J.~Cordero,$^{45}$
J.~Prat,$^{22,46}$
J.~Myles,$^{3}$
K.~Eckert,$^{29}$
K.~Bechtol,$^{47}$
K.~Herner,$^{23}$
L.~F.~Secco,$^{24}$
M.~Gatti,$^{29}$
M.~Raveri,$^{48}$
M.~Carrasco~Kind,$^{49,50}$
M.~R.~Becker,$^{20}$
M.~A.~Troxel,$^{51}$
M.~Jarvis,$^{29}$
N.~MacCrann,$^{52}$
O.~Friedrich,$^{53}$
O.~Alves,$^{12}$
P.-F.~Leget,$^{16}$
R.~Chen,$^{51}$
R.~P.~Rollins,$^{45}$
R.~H.~Wechsler,$^{54,16,17}$
R.~A.~Gruendl,$^{49,50}$
R.~Cawthon,$^{55}$
S.~Allam,$^{23}$
S.~L.~Bridle,$^{45}$
S.~Pandey,$^{29}$
S.~Everett,$^{32}$
T.~Shin,$^{56}$
W.~G.~Hartley,$^{57}$
X.~Fang,$^{58,36}$
Y.~Zhang,$^{59}$
M.~Aguena,$^{18}$
J.~Annis,$^{23}$
D.~Bacon,$^{60}$
E.~Bertin,$^{61,62}$
S.~Bocquet,$^{31}$
D.~Brooks,$^{63}$
J.~Carretero,$^{35}$
F.~J.~Castander,$^{64,21}$
L.~N.~da Costa,$^{18}$
M.~E.~S.~Pereira,$^{65}$
J.~De~Vicente,$^{39}$
S.~Desai,$^{66}$
P.~Doel,$^{63}$
I.~Ferrero,$^{67}$
B.~Flaugher,$^{23}$
J.~Frieman,$^{23,24}$
J.~Garc\'ia-Bellido,$^{68}$
E.~Gaztanaga,$^{64,60,21}$
G.~Gutierrez,$^{23}$
S.~R.~Hinton,$^{69}$
D.~L.~Hollowood,$^{70}$
K.~Honscheid,$^{27,71}$
D.~Huterer,$^{12}$
D.~J.~James,$^{72}$
K.~Kuehn,$^{73,74}$
O.~Lahav,$^{63}$
S.~Lee,$^{32}$
J.~L.~Marshall,$^{75}$
J. Mena-Fern{\'a}ndez,$^{76}$
R.~Miquel,$^{77,35}$
J.~Muir,$^{78}$
M.~Paterno,$^{23}$
A.~A.~Plazas~Malag\'on,$^{16,17}$
A.~Porredon,$^{79}$
A.~K.~Romer,$^{80}$
S.~Samuroff,$^{43}$
E.~Sanchez,$^{39}$
D.~Sanchez Cid,$^{39}$
M.~Smith,$^{81}$
M.~Soares-Santos,$^{82,12}$
E.~Suchyta,$^{83}$
M.~E.~C.~Swanson,$^{49}$
G.~Tarle,$^{12}$
C.~To,$^{27}$
N.~Weaverdyck,$^{58,44}$
J.~Weller,$^{84,85}$
P.~Wiseman,$^{81}$
and M.~Yamamoto$^{51}$
\begin{center} (DES Collaboration) \end{center}
}
\vspace{0.4cm}
\\
\parbox{\textwidth}{
%\scriptsize
$^{1}$ Institute of Astronomy, University of Cambridge, Madingley Road, Cambridge CB3 0HA, UK\\
$^{2}$ Kavli Institute for Cosmology Cambridge, Madingley Road, Cambridge, CB3 OHA\\
$^{3}$ Department of Astrophysical Sciences, Princeton University, Peyton Hall, Princeton, NJ 08544, USA\\
$^{4}$ Institute for Computational Science, University of Zurich, Winterthurerstrasse 190, CH-8057 Zurich, Switzerland\\
$^{5}$ Astrophysics Research Institute, Liverpool John Moores University, 146 Brownlow Hill, Liverpool L3 5RF, UK\\
$^{6}$ Centre for Energy, Environmental and Technological Research, Av. Complutense, 40, Moncloa - Aravaca, 28040 Madrid, Spain\\
$^{7}$ Kavli Institute for Particle Astrophysics and Cosmology,
382 Via Pueblo Mall Stanford, CA 94305-4060, USA\\
$^{8}$ SLAC National Accelerator Laboratory 2575 Sand Hill Road Menlo Park, California 94025, USA\\
$^{9}$ Physics Division, Lawrence Berkeley National Laboratory, Berkeley, CA 94720, USA\\
$^{10}$ Berkeley Center for Cosmological Physics, Department of Physics,
University of California, Berkeley, CA 94720, USA\\
$^{11}$  Department of Astronomy, Cornell University, Ithaca, NY 14853, USA\\
$^{12}$ Department of Physics, University of Michigan, Ann Arbor, MI 48109, USA\\
$^{13}$ Kavli Institute for the Physics and Mathematics of the Universe (WPI), UTIAS, The University of Tokyo, Kashiwa, Chiba 277-8583, Japan\\
$^{14}$ Department of Physics, Carnegie Mellon University, Pittsburgh, Pennsylvania 15312, USA\\
$^{15}$ NSF AI Planning Institute for Physics of the Future, Carnegie Mellon University, Pittsburgh, PA 15213, USA\\
$^{16}$ Kavli Institute for Particle Astrophysics \& Cosmology, P. O. Box 2450, Stanford University, Stanford, CA 94305, USA\\
$^{17}$ SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA\\
$^{18}$ Laborat\'orio Interinstitucional de e-Astronomia - LIneA, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil\\
$^{19}$ Observat\'orio Nacional, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil\\
$^{20}$ Argonne National Laboratory, 9700 South Cass Avenue, Lemont, IL 60439, USA\\
$^{21}$ Institute of Space Sciences (ICE, CSIC),  Campus UAB, Carrer de Can Magrans, s/n,  08193 Barcelona, Spain\\
$^{22}$ Department of Astronomy and Astrophysics, University of Chicago, Chicago, IL 60637, USA\\
$^{23}$ Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA\\
$^{24}$ Kavli Institute for Cosmological Physics, University of Chicago, Chicago, IL 60637, USA\\
$^{25}$ NASA Goddard Space Flight Center, 8800 Greenbelt Rd, Greenbelt, MD 20771, USA\\
$^{26}$ Instituto de F\'isica Gleb Wataghin, Universidade Estadual de Campinas, 13083-859, Campinas, SP, Brazil\\
$^{27}$ Center for Cosmology and Astro-Particle Physics, The Ohio State University, Columbus, OH 43210, USA\\
$^{28}$ Instituto de Astrofisica de Canarias, E-38205 La Laguna, Tenerife, Spain\\
$^{29}$ Department of Physics and Astronomy, University of Pennsylvania, Philadelphia, PA 19104, USA\\
$^{30}$ Universit\'e Grenoble Alpes, CNRS, LPSC-IN2P3, 38000 Grenoble, France\\
$^{31}$ University Observatory, Faculty of Physics, Ludwig-Maximilians-Universit\"at, Scheinerstr. 1, 81679 Munich, Germany\\
$^{32}$ Jet Propulsion Laboratory, California Institute of Technology, 4800 Oak Grove Dr., Pasadena, CA 91109, USA\\
$^{33}$ Brookhaven National Laboratory, Bldg 510, Upton, NY 11973, USA\\
$^{34}$ Department of Physics, ETH Zurich, Wolfgang-Pauli-Strasse 16, CH-8093 Zurich, Switzerland\\
$^{35}$ Institut de F\'{\i}sica d'Altes Energies (IFAE), The Barcelona Institute of Science and Technology, Campus UAB, 08193 Bellaterra (Barcelona) Spain\\
$^{36}$ Department of Astronomy/Steward Observatory, University of Arizona, 933 North Cherry Avenue, Tucson, AZ 85721-0065, USA\\
$^{37}$ Department of Physics, University of Arizona, Tucson, AZ 85721, USA\\
$^{38}$ School of Physics and Astronomy, Cardiff University, CF24 3AA, UK\\
$^{39}$ Centro de Investigaciones Energ\'eticas, Medioambientales y Tecnol\'ogicas (CIEMAT), Madrid, Spain\\
$^{40}$ Institut de Recherche en Astrophysique et Plan\'etologie (IRAP), Universit\'e de Toulouse, CNRS, UPS, CNES, 14 Av. Edouard Belin, 31400 Toulouse, France\\
$^{41}$ Department of Physics and Astronomy, University of Waterloo, 200 University Ave W, Waterloo, ON N2L 3G1, Canada\\
$^{42}$ Institute for Astronomy, University of Edinburgh, Edinburgh EH9 3HJ, UK\\
$^{43}$ Department of Physics, Northeastern University, Boston, MA 02115, USA\\
$^{44}$ Lawrence Berkeley National Laboratory, 1 Cyclotron Road, Berkeley, CA 94720, USA\\
$^{45}$ Jodrell Bank Center for Astrophysics, School of Physics and Astronomy, University of Manchester, Oxford Road, Manchester, M13 9PL, UK\\
$^{46}$ Nordita, KTH Royal Institute of Technology and Stockholm University, Hannes Alfv\'ens v\"ag 12, SE-10691 Stockholm, Sweden\\
$^{47}$ Physics Department, 2320 Chamberlin Hall, University of Wisconsin-Madison, 1150 University Avenue Madison, WI  53706-1390\\
$^{48}$ Department of Physics, University of Genova and INFN, Via Dodecaneso 33, 16146, Genova, Italy\\
$^{49}$ Center for Astrophysical Surveys, National Center for Supercomputing Applications, 1205 West Clark St., Urbana, IL 61801, USA\\
$^{50}$ Department of Astronomy, University of Illinois at Urbana-Champaign, 1002 W. Green Street, Urbana, IL 61801, USA\\
$^{51}$ Department of Physics, Duke University Durham, NC 27708, USA\\
$^{52}$ Department of Applied Mathematics and Theoretical Physics, University of Cambridge, Cambridge CB3 0WA, UK\\
$^{53}$ Kavli Institute for Cosmology, University of Cambridge, Madingley Road, Cambridge CB3 0HA, UK\\
$^{54}$ Department of Physics, Stanford University, 382 Via Pueblo Mall, Stanford, CA 94305, USA\\
$^{55}$ Physics Department, William Jewell College, Liberty, MO, 64068\\
$^{56}$ Department of Physics and Astronomy, Stony Brook University, Stony Brook, NY 11794, USA\\
$^{57}$ Department of Astronomy, University of Geneva, ch. d'\'Ecogia 16, CH-1290 Versoix, Switzerland\\
$^{58}$ Department of Astronomy, University of California, Berkeley,  501 Campbell Hall, Berkeley, CA 94720, USA\\
$^{59}$ Cerro Tololo Inter-American Observatory, NSF's National Optical-Infrared Astronomy Research Laboratory, Casilla 603, La Serena, Chile\\
$^{60}$ Institute of Cosmology and Gravitation, University of Portsmouth, Portsmouth, PO1 3FX, UK\\
$^{61}$ CNRS, UMR 7095, Institut d'Astrophysique de Paris, F-75014, Paris, France\\
$^{62}$ Sorbonne Universit\'es, UPMC Univ Paris 06, UMR 7095, Institut d'Astrophysique de Paris, F-75014, Paris, France\\
$^{63}$ Department of Physics \& Astronomy, University College London, Gower Street, London, WC1E 6BT, UK\\
$^{64}$ Institut d'Estudis Espacials de Catalunya (IEEC), 08034 Barcelona, Spain\\
$^{65}$ Hamburger Sternwarte, Universit\"{a}t Hamburg, Gojenbergsweg 112, 21029 Hamburg, Germany\\
$^{66}$ Department of Physics, IIT Hyderabad, Kandi, Telangana 502285, India\\
$^{67}$ Institute of Theoretical Astrophysics, University of Oslo. P.O. Box 1029 Blindern, NO-0315 Oslo, Norway\\
$^{68}$ Instituto de Fisica Teorica UAM/CSIC, Universidad Autonoma de Madrid, 28049 Madrid, Spain\\
$^{69}$ School of Mathematics and Physics, University of Queensland,  Brisbane, QLD 4072, Australia\\
$^{70}$ Santa Cruz Institute for Particle Physics, Santa Cruz, CA 95064, USA\\
$^{71}$ Department of Physics, The Ohio State University, Columbus, OH 43210, USA\\
$^{72}$ Center for Astrophysics $\vert$ Harvard \& Smithsonian, 60 Garden Street, Cambridge, MA 02138, USA\\
$^{73}$ Australian Astronomical Optics, Macquarie University, North Ryde, NSW 2113, Australia\\
$^{74}$ Lowell Observatory, 1400 Mars Hill Rd, Flagstaff, AZ 86001, USA\\
$^{75}$ George P. and Cynthia Woods Mitchell Institute for Fundamental Physics and Astronomy, and Department of Physics and Astronomy, Texas A\&M University, College Station, TX 77843,  USA\\
$^{76}$ LPSC Grenoble - 53, Avenue des Martyrs 38026 Grenoble, France\\
$^{77}$ Instituci\'o Catalana de Recerca i Estudis Avan\c{c}ats, E-08010 Barcelona, Spain\\
$^{78}$ Perimeter Institute for Theoretical Physics, 31 Caroline St. North, Waterloo, ON N2L 2Y5, Canada\\
$^{79}$ Ruhr University Bochum, Faculty of Physics and Astronomy, Astronomical Institute, German Centre for Cosmological Lensing, 44780 Bochum, Germany\\
$^{80}$ Department of Physics and Astronomy, Pevensey Building, University of Sussex, Brighton, BN1 9QH, UK\\
$^{81}$ School of Physics and Astronomy, University of Southampton,  Southampton, SO17 1BJ, UK\\
$^{82}$ \\
$^{83}$ Computer Science and Mathematics Division, Oak Ridge National Laboratory, Oak Ridge, TN 37831\\
$^{84}$ Max Planck Institute for Extraterrestrial Physics, Giessenbachstrasse, 85748 Garching, Germany\\
$^{85}$ Universit\"ats-Sternwarte, Fakult\"at f\"ur Physik, Ludwig-Maximilians Universit\"at M\"unchen, Scheinerstr. 1, 81679 M\"unchen, Germany\\
}
}

